How Effective is Multiple-Vantage-Point Domain Control Validation?

Multiple-vantage-point domain control validation (multiVA) is an emerging defense for mitigating BGP hijacking attacks against certificate authorities. While the adoption of multiVA is on the rise, little work has quantified its effectiveness against BGP hijacks in the wild. We bridge the gap by presenting the first analysis framework that measures the security of a multiVA deployment under real-world network configurations (e.g., DNS and RPKI). Our framework accurately models the attack surface of multiVA by 1) considering the attacks on DNS nameservers involved in domain validation, 2) considering deployed practical security techniques such as RPKI, 3) performing fine-grained internet-scale analysis to compute multiVA resilience (i.e., how difficult it is to launch a BGP hijack against a domain and get a bogus certificate under multiVA). We use our framework to perform a rigorous security analysis of the multiVA deployment of Let's Encrypt, using a dataset that consists of about 1 million certificates and 31 billion DNS queries collected over four months. Our analysis shows while DNS does enlarge the attack surface of multiVA, the of Let's Encrypt's multiVA deployment still offers an 88% median resilience against BGP hijacks, a notable improvement over 76% offered by single-vantage-point validation. RPKI, even in its current state of partial deployment, effectively mitigates BGP attacks and improves the security of the deployment by 15% as compared to the case without considering RPKI. Exploring 11,000 different multiVA configurations, we find that Let's Encrypt's deployment can be further enhanced to achieve a resilience of over 99% by using a full quorum policy with only two additional vantage points in different public clouds.

==> sections/add_results.tex <==
\section{Results Still To Cover}
\subsection{The impact of nameserver selection on resilience}

\subsubsection{Impact of CDN Geographic Load Balancing} If we use lookups from a different region, how does resilience change? What fraction of domains are affected by this.

\begin{tabular}{|c|c|}
    \hline
    region & average num. target DNS addresses \\
    us-east-2 & 7.08 \\
    \hline
    ap-southeast-1 & 7.095 \\
    \hline
    ap-northeast-1 & 7.10 \\
    \hline
    eu-west-3 & 7.117 \\
    \hline
    eu-central-1 & 7.147 \\
    \hline
    us-west-2 & 7.42 \\
    \hline
\end{tabular}

\subsubsection{Impact of DNSSEC}
Does the root and TLDs being DNSSEC signed actually make a difference? How big is their attack surface (particularly since they are aggressively anycast). Can we get anywhere interesting with DNSSEC cross chain trust?
Some other ideas: distribution of DNSSEC by TLD, by region

\subsubsection{Glueless Lookups}
Are glueless DNS records really a big problem? How many domains are affected and what is the affect on resilience. Are there any particular providers that are super bad. Henry note: remind Grace to consider list of only nameserver (no glugless) IPs in summary statistics file.

\henry{in other words: how often do glueless lookups happen? how do they change attack surface?}

\subsection{DNS profiling of Let's Encrypt domains} How centralized is the DNS ecosystem of Let's Encrypt domains? Can we potentially focus resilience improvement on just a couple providers?
Distribution of hosting providers, geographical location of nameservers
